AuxDet: Auxiliary Metadata Matters for Omni-Domain Infrared Small Target Detection

Omni-domain infrared small target detection (Omni-IRSTD) poses formidable challenges, as a single model must seamlessly adapt to diverse imaging systems, varying resolutions, and multiple spectral bands simultaneously. Current approaches predominantly rely on visual-only modeling paradigms that not only struggle with complex background interference and inherently scarce target features, but also exhibit limited generalization capabilities across complex omni-scene environments where significant domain shifts and appearance variations occur. In this work, we reveal a critical oversight in existing paradigms: the neglect of readily available auxiliary metadata describing imaging parameters and acquisition conditions, such as spectral bands, sensor platforms, resolution, and observation perspectives. To address this limitation, we propose the Auxiliary Metadata Driven Infrared Small Target Detector (AuxDet), a novel multimodal framework that is the first to incorporate metadata into the IRSTD paradigm for scene-aware optimization. Through a high-dimensional fusion module based on multi-layer perceptrons (MLPs), AuxDet dynamically integrates metadata semantics with visual features, guiding adaptive representation learning for each individual sample. Additionally, we design a lightweight prior-initialized enhancement module using 1D convolutional blocks to further refine fused features and recover fine-grained target cues. Extensive experiments on the challenging WideIRSTD-Full benchmark demonstrate that AuxDet consistently outperforms state-of-the-art methods, validating the critical role of auxiliary information in improving robustness and accuracy in omni-domain IRSTD tasks. Code is available at https://github.com/GrokCV/AuxDet.

==> journal-contents/9-biography.tex <==
% !TEX root = ../main.tex

\newpage

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{journal_figs/biography/Yangting_shi}}]{Yangting Shi}
is currently pursuing a Master’s degree in the School of Electronics and Information at Northwestern Polytechnical University, where she also completed her undergraduate studies. She is also a research intern at VCIP, Nankai University, supervised by Prof. Yimian Dai. Her research interests primarily focus on infrared small target detection.
\vspace{-4mm}
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{journal_figs/biography/Mengze_Xu}}]{Mengze Xu}
is currently pursuing the M.E. degree at the College of Computer Science, Nankai University, supervised by Prof. Yimian Dai. He received the B.E. degree from Beijing Foreign Studies University in 2024. His research interests focus on Infrared Small Target Detection.
\vspace{-4mm}
\end{IEEEbiography}

% Renjie He
\begin{IEEEbiography}[{\includegraphics[width=1.1in,height=1.35in,clip,keepaspectratio]{journal_figs/biography/Renjie_He}}]{Renjie He} (Member, IEEE) received the Ph.D. degree in signal and information processing from Northwestern Polytechnical University (NPU) in 2017. From 2017 to 2020, he was a Research Fellow with Nanyang Technological University, Singapore. He is currently an Associate Professor of Northwestern Polytechnical University. He has published over 30 papers in IEEE Transactions on Industrial Electronics (TIE), IEEE Transactions on Geoscience and Remote Sensing (TGRS), Sensors, APSIPA Transactions on Signal and Information Processing (TSIP), International Conference on Acoustics, Speech and Signal Processing (ICASSP), Asia-Pacific Signal and Information Processing Association (APSIPA), and IEEE International Conference on Industrial Engineering and Applications (ICIEA). His research interests include low-level computer vision, deep learning, and RS image processing with applications to industry and digital protection of cultural heritage.
\end{IEEEbiography}

% Le Hui
\begin{IEEEbiography}[{\includegraphics[width=1.1in,height=1.35in,clip,keepaspectratio]{journal_figs/biography/Le_Hui}}]{Le Hui} received the Ph.D. degree from the School of Computer Science and Engineering, Nanjing University of Science and Technology (NUST), Nanjing, China, in 2022. He is currently a Associate Professor at the Northwestern Polytechnical University (NWPU), Xi’an, China. His current research interests include 3D point cloud processing, such as semantic segmentation, single object tracking, place recognition, and point cloud generation.
\end{IEEEbiography}

% Xiang Li
\begin{IEEEbiography}[{\includegraphics[width=1.1in,height=1.35in,clip,keepaspectratio]{journal_figs/biography/Xiang_Li}}]{Xiang Li} is an Associate Professor in College of Computer Science, Nankai University. He received the PhD degree from the Department of Computer Science and Technology, Nanjing University of Science and Technology (NJUST) in 2020. There, he started the postdoctoral career in NJUST as a candidate for the 2020 Postdoctoral Innovative Talent Program. In 2016, he spent 8 months as a research intern in Microsoft Research Asia, supervised by Prof. Tao Qin and Prof. Tie-Yan Liu. He was a visiting scholar at Momenta, mainly focusing on monocular perception algorithm. His recent works are mainly on: neural architecture design, CNN/Transformer, object detection/recognition, unsupervised learning, and knowledge distillation. He has published 20+ papers in top journals and conferences such as TPAMI, CVPR, NeurIPS, etc.
\end{IEEEbiography}

% Jian Yang
\begin{IEEEbiography}[{
  \includegraphics[width=1.45in,height=1.3in,clip,keepaspectratio]{journal_figs/biography/Jian_Yang}}]{Jian Yang} received the PhD degree from Nanjing University of Science and Technology (NJUST) in 2002, majoring in pattern recognition and intelligence systems. From 2003 to 2007, he was a Postdoctoral Fellow at the University of Zaragoza, Hong Kong Polytechnic University and New Jersey Institute of Technology, respectively. From 2007 to present, he is a professor in the School of Computer Science and Technology of NJUST. Currently, he is also a visiting distinguished professor in the College of Computer Science of Nankai University. He is the author of more than 300 scientific papers in pattern recognition and computer vision. His papers have been cited over 40000 times in the Scholar Google. His research interests include pattern recognition and computer vision. Currently, he is/was an associate editor of Pattern Recognition, Pattern Recognition Letters, IEEE Trans. Neural Networks and Learning Systems, and Neurocomputing. He is a Fellow of IAPR. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{journal_figs/biography/Mingming_Cheng}}]{Ming-Ming Cheng}
 received his PhD degree from Tsinghua University in 2012. Then, he did 2 years research fellow, with Prof. Philip Torr in Oxford. He is now a professor at Nankai University, leading the Media Computing Lab. His research interests include computer graphics, computer vision, and image processing. He received research awards, including the National Science Fund for Distinguished Young Scholars and the ACM China Rising Star Award. He is on the editorial boards of IEEE TPAMI and IEEE TIP.
\vspace{-4mm}
\end{IEEEbiography}

% Yimian Dai
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{journal_figs/biography/Yimian_Dai}}]{Yimian Dai}
(Member, IEEE) received the B.E. degree in information engineering and the Ph.D. degree in signal and information processing from Nanjing University of Aeronautics and Astronautics, Nanjing, China, in 2013 and 2020, respectively.
From 2021 to 2024, he was a Postdoctoral Researcher with the School of Computer Science and Engineering, Nanjing University of Science and Technology, Nanjing, China. 
He is currently an Associate Professor with the College of Computer Science, Nankai University, Tianjin, China.
His research interests include computer vision, deep learning, and their applications in remote sensing.
For more information, please visit the link (\href{https://yimian.grokcv.ai/}{https://yimian.grokcv.ai/}).
% (Member, IEEE) received the B.S. and Ph.D. degrees in signal and information processing from Nanjing University of Aeronautics and Astronautics (NUAA), Nanjing, China, in 2013 and 2021, respectively.
% From 2021 to 2024, he was a Postdoctoral Researcher with the School of Computer Science and Engineering, Nanjing University of Science and Technology (NJUST), Nanjing, China. During his Ph.D. study, he was a visiting scholar at the Department of Computer Science, University of Copenhagen, Denmark, under the supervision of Prof. Fabian Gieseke from March 2018 to September 2018, and at the Department of Computer Science, University of Arizona, USA, under the supervision of Prof. Kobus Barnard from October 2018 to October 2020.

% Since 2025, he has been an Associate Professor with the College of Computer Science, Nankai University, Tianjin, China. His research interests include computer vision, deep learning, and their applications in remote sensing, with a particular focus on developing advanced object detection algorithms to address real-world challenges.
% received his Ph.D. in signal and information processing from Nanjing University of Aeronautics and Astronautics in 2021. During his doctoral studies, he was a visiting Ph.D. student at the University of Copenhagen from March 2018 to September 2018, and at the University of Arizona from October 2018 to October 2020. He is currently an assistant researcher at Nanjing University of Science and Technology, where his research focuses on remote sensing, computer vision, and deep learning.
\end{IEEEbiography}
